Evaporative cooling of cold atoms at surfaces

We theoretically investigate the evaporative cooling of cold rubidium atoms that are brought close to a solid surface. The dynamics of the atom cloud are described by coupling a dissipative Gross-Pitaevskii equation for the condensate with a quantum Boltzmann description of the thermal cloud (the Zaremba-Nikuni-Griffin method). We have also performed experiments to allow for a detailed comparison with this model and find that it can capture the key physics of this system provided the full collisional dynamics of the thermal cloud are included. In addition, we suggest how to optimize surface cooling to obtain the purest and largest condensates.

==> header.tex <==
\RequirePackage[utf8]{inputenc}

\usepackage{amsmath}
\usepackage{graphics}

